Enhance transferability of adversarial examples with model architecture

Transferability of adversarial examples is of critical importance to launch black-box adversarial attacks, where attackers are only allowed to access the output of the target model. However, under such a challenging but practical setting, the crafted adversarial examples are always prone to overfitting to the proxy model employed, presenting poor transferability. In this paper, we suggest alleviating the overfitting issue from a novel perspective, i.e., designing a fitted model architecture. Specifically, delving the bottom of the cause of poor transferability, we arguably decompose and reconstruct the existing model architecture into an effective model architecture, namely multi-track model architecture (MMA). The adversarial examples crafted on the MMA can maximumly relieve the effect of model-specified features to it and toward the vulnerable directions adopted by diverse architectures. Extensive experimental evaluation demonstrates that the transferability of adversarial examples based on the MMA significantly surpass other state-of-the-art model architectures by up to 40% with comparable overhead.

==> tex/related_work.tex <==
\subsection{Adversarial Attack}
Adversarial attack aims to produce adversarial examples to fool the target model by slightly perturbing images, and existing methods can be generally divided two categories based on the knowledge of attackers: white-box attack and black-box attack.
\par
\textbf{White-box attack.}
In the white-box setting, the attackers commonly adopt an optimization method in input space to increase loss for producing adversarial examples.
Besides, such methods also is the foundation of transfer-based attack, and we give a brief review to classic white-box attack methods as following.
As the seminal work of this area, FGSM \cite{} perturbs the clean seed images for one step along with the sign of the gradient of the loss.
Compared to it, basic iterative method (BIM) \cite{} extends FGSM with multi-step to craft adversarial examples.
Realizing the drawback of adversarial examples being easily trapping local minima, projected gradient descent (PGD) \cite{} add random noises into the seed images for escaping the local minima.
Carlini and Wagner attack (C\&W) \cite{} designed a brilliant loss function, which successfully broke several defense methods, e.g., defensive knowledge distillation.
\par
\textbf{Black-box attack.}
We mainly review the technologies of increasing transferability of adversarial examples.
For transfer-based adversarial attack, attackers launch attacks on the plug-and-play proxy model adopting white-box attack methods, such as FGSM, PGD.
Unfortunately, the vanilla method commonly shows lower success due to overfit to specific features of the proxy model, which was revealed by \cite{}.
To generate adversarial examples with high transferability, the shared low-level features over diverse model is the critical factor.
\par
From the model perspective, Ensemble attack (EA), proposed by \cite{}, is a straightforward method, where a adversarial instance is generated by ensembling multiple model.
Dispite the EA captures the more low-level features, it suffers from huge computation cost.
Another approach of focusing the model is skip gradient method (SGM) \cite{}, where a decay factor is applied into the skip connections for forcing the model to pay more attention in low-level features.
\par
From the optimizer perspective, \cite{} proposed momentum iterative boosting (MI) that incorporating a momentum term into the attack method (i.e., momentum optimizer) can boost the transferability. 
Further, \cite{} extended the MI with displacing momentum optimizer as nesterov optimizer.
\par
From the data perspective, \cite{} proposed diversity input (DI) strategy to mitigate the overfitting problem, where the random transformations is applied to the input images at each iteration.
Similar to DI, translation invariant (TI) \cite{} suggested that the crafted adversarial examples should be non-sensitive to the discriminative regions of the proxy model.

\subsection{Adversarial Defense}
To mitigate the threat of adversarial attacks, various defense methods have been proposed.
However, the effectiveness of most of such methods stems from obfuscated gradients (e.g., defensive knowledge distillation), which is easily broken as shown in \cite{} except adversarial training.
Till now, adversarial training (AT) is believed to be the most robust and reliable method and its basic idea is feeding the crafted adversarial examples with normal examples into the model for training.
The study of adversarial examples mainly lies in two aspects: increasing efficiency of AT \cite{} and enhancing robustness of the model with AT \cite{}.
